PersonaBooth: Personalized Text-to-Motion Generation

This paper introduces Motion Personalization, a new task that generates personalized motions aligned with text descriptions using several basic motions containing Persona. To support this novel task, we introduce a new large-scale motion dataset called PerMo (PersonaMotion), which captures the unique personas of multiple actors. We also propose a multi-modal finetuning method of a pretrained motion diffusion model called PersonaBooth. PersonaBooth addresses two main challenges: i) A significant distribution gap between the persona-focused PerMo dataset and the pretraining datasets, which lack persona-specific data, and ii) the difficulty of capturing a consistent persona from the motions vary in content (action type). To tackle the dataset distribution gap, we introduce a persona token to accept new persona features and perform multi-modal adaptation for both text and visuals during finetuning. To capture a consistent persona, we incorporate a contrastive learning technique to enhance intra-cohesion among samples with the same persona. Furthermore, we introduce a context-aware fusion mechanism to maximize the integration of persona cues from multiple input motions. PersonaBooth outperforms state-of-the-art motion style transfer methods, establishing a new benchmark for motion personalization.

==> table/Yihua_comp_Method.tex <==

\begin{table}[t]
    \setlength\tabcolsep{6pt}
    \renewcommand\arraystretch{1.2}
    
    \small
    \caption{Comparison of motion generation tasks. (Feel free to Delete}
    
    \centering
    \begin{tabular}{lcccc}
    \toprule[1pt]
    
      \multirow{2}{*}{Motion Task} & \multicolumn{2}{c}{Conditions}&  \multirow{2}{*}{\makecell{Multi\\Modal}}  & \multirow{2}{*}{\makecell{Motion\\Prompts}} \\
      \cline{2-3}
     & Text & Motion & \\
    \hline    
    Generation~\cite{zhang2022motiondiffuse,chen2023executing} & \gcheck & \rx &\rx& None 
    \\
    Style Transfer~\cite{raab2024monkey,zhong2024smoodi} & \rx& $\gcheck$&\rx&Single \\ 
    \hline
    
    Personalization (Ours) & \gcheck& \gcheck&\gcheck&Multiple\\
    \bottomrule[1pt]
    \end{tabular}
  
\end{table}

==> table/abl_old.tex <==
\begin{table}[t]

\caption{Ablation study of the proposed components. The top three rows show results for single-input (SI) cases, while the last two rows are for multiple-input (MI) cases}
\label{tab:abl}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule[1pt]
\multirow{2}{*}{Methods} & \multirow{2}{*}{FID $\downarrow$} &\multicolumn{3}{c}{R Precision $\uparrow$} & \multirow{2}{*}{SRA avg.$\uparrow$} & \multirow{2}{*}{Diversity $\uparrow$} \\ \cmidrule(lr){3-5}
 & & \multicolumn{1}{c}{Top 1} & \multicolumn{1}{c}{Top 2} & \multicolumn{1}{c}{Top 3} & & \\\midrule 
  \textit{SI}\; baseline &
  7.45 &
  0.06 &
  0.11 &
  0.16 &
  17.99 &
  7.48
\\
  \textit{SI}\; \; + $P^*$  &
   5.06 &
   0.05 &
   0.10 &
   0.15 &
   18.26 &
   8.01 
\\
  \textit{SI}\; \;\quad +$L_{pc}$ &
   3.14 &
   0.15 &
   0.25 &
   0.33 &
   18.05 &
   7.80
\\\midrule
  \textit{MI}\; Mean &
  3.52 &
  \textbf{0.19} &
  \textbf{0.30} &
  0.38 &
  \textbf{19.24} &
  7.88
\\
  \textit{MI}\; CAF &
  \textbf{2.95} &
  \textbf{0.19} &
  \textbf{0.30} &
  \textbf{0.39} &
  18.13 &
  \textbf{8.12}
\\ \bottomrule[1pt]
\end{tabular}%
}

\end{table}


==> table/comp_PerMo_old.tex <==
\begin{table*}[t]

\caption{Comparison with the state-of-the-art methods on the PerMo dataset. PersonaBooth (SI) and PersonaBooth (MI) indicate our complete model for single inputs and multiple inputs, respectively. 
MCM-LDM* indicates the model is finetuned on the PerMo dataset. 
The second-highest values are underlined}
\label{tab:comp_PerMo}
\vspace{-0.6cm}
\center
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llcccccccccccccccc@{}}
\toprule[1pt]
\multirow{2}{*}{Methods} & \multirow{2}{*}{Steps} & \multirow{2}{*}{FID $\downarrow$} &\multicolumn{3}{c}{R Precision $\uparrow$}  & \multicolumn{10}{c}{SRA $\uparrow$} & \multirow{2}{*}{Diversity $\uparrow$} \\ \cmidrule(lr){4-6} \cmidrule(lr){7-16}
 &  &  &
 \multicolumn{1}{c}{Top 1} &
 \multicolumn{1}{c}{Top 2} &
 \multicolumn{1}{c}{Top 3} &
 \multicolumn{1}{c}{Age} &
 \multicolumn{1}{c}{Char1} &
 \multicolumn{1}{c}{Char2} &
 \multicolumn{1}{c}{Cond1} &
 \multicolumn{1}{c}{Cond2} &
 \multicolumn{1}{c}{Emo1} &
 \multicolumn{1}{c}{Emo2} &
 \multicolumn{1}{c}{Trait} &
 \multicolumn{1}{c}{Sur} &
 \multicolumn{1}{c}{\textbf{Avg.}}
 &
 \\\midrule 
 
  MoMo~\cite{raab2024monkey}&
  100 &
  13.91 &
  0.05 &
  0.09 &
  0.13 &
  28.23 &
  10.23 &
  11.30 &
  \textbf{8.73} &
  15.97 &
  9.97 &
  14.57 &
  12.60 &
  7.93 &
  13.47 &
  6.74
\\
  MCM-LDM~\cite{song2024arbitrary}&
  1000 &
  9.16 &
  0.13 &
  0.23 &
  0.30 &
  47.38 &
  11.44 &
  10.34 &
  7.63 &
  18.90 &
  11.69 &
  17.20 &
  \underline{15.71} &
  \underline{9.22} &
  17.00 &
  6.70
\\
  MCM-LDM*~\cite{song2024arbitrary} &
  1000 &
  9.70 &
  0.13 &
  0.23 &
  0.30 &
  46.49 &
  12.12 &
  9.22 &
  \underline{7.95} &
  \underline{19.77} &
  \underline{11.75} &
  18.05 &
  15.18 &
  7.33 &
  16.76 &
  6.76
\\\midrule
  PersonaBooth (SI) &
  50 &
  \underline{3.14} &
  \underline{0.15} &
  \underline{0.25} &
  \underline{0.33} &
  \underline{48.00} &
  \underline{13.67} &
  \underline{11.97} &
  6.69 &
  18.67 &
  \textbf{14.34} &
  \textbf{19.75} &
  \textbf{17.06} &
  8.80 &
  \underline{18.05} &
  \underline{7.80}
\\
  PersonaBooth (MI) &
  50 &
  \textbf{2.95} &
  \textbf{0.19} &
  \textbf{0.30} &
  \textbf{0.39} &
  \textbf{51.95} &
  \textbf{14.89} &
  \textbf{12.00} &
  5.16 &
  \textbf{22.95} &
  9.44 &
  \underline{18.14} &
  15.45 &
  \textbf{10.09} &
  \textbf{18.13} &
  \textbf{8.12}
  
\\ \bottomrule[1pt]
\end{tabular}%
}

\end{table*}


==> table/dataset.tex <==
\begin{table}[t]
\caption{Comparison with existing motion style datasets. The note for `*' is provided in the main text. `-' indicates no information provided}
\label{tab:dataset}

\resizebox{\linewidth}{!}{%
\centering

\begin{tabular}{l|c|c|c|c|c|c}
\toprule[1pt]
Dataset & Actors & Styles & Contents & Clips & Mesh & Text\\ \midrule
    Xia \cite{xia2015realtime}&
    - &
    8 &
    9 &
    572 &
    \rx &
    \rx \\
    BFA \cite{aberman2020unpaired}&
    1 &
    16 &
    9 &
    32 &
    \rx &
    \rx  \\
    BN-1 \cite{kobayashi2023motion}&
    2* &
    15 &
    17 &
    175 &
    \rx &
    \rx  \\
    BN-2 \cite{kobayashi2023motion}&
    2* &
    7 &
    10 &
    2,902 &
    \rx &
    \rx  \\
    100Style \cite{mason2022real}&
    1 &
    100* &
    8* &
    810 &
    \rx &
    \rx  \\ \midrule
    \textbf{PerMo} &
    5 &
    34 &
    10 &
    6,610 &
    \gcheck &
    \gcheck\\
\bottomrule[1pt]    
\end{tabular}
}
\end{table}
